Dynamic Budget Management with Service Guarantees for Mixed-Criticality Systems

Many existing studies on mixed-criticality (MC) scheduling assume that low-criticality budgets for high-criticality applications are known apriori. These budgets are primarily used as guidance to determine when the scheduler should switch the system mode from low to high. Based on this key observation, in this paper we propose a dynamic MC scheduling model under which low-criticality budgets for individual high-criticality applications are determined at runtime as opposed to being fixed offline. To ensure sufficient budget for high-criticality applications at all times, we use offline schedulability analysis to determine a system-wide total low-criticality budget allocation for all the high-criticality applications combined. This total budget is used as guidance in our model to determine the need for a mode-switch. The runtime strategy then distributes this total budget among the various applications depending on their execution requirement and with the objective of postponing mode-switch as much as possible. We show that this runtime strategy is able to postpone mode-switches for a longer time than any strategy that uses a fixed low-criticality budget allocation for each application. Finally, since we are able to control the total budget allocation for high-criticality applications before mode-switch, we also propose techniques to determine these budgets considering system-wide objectives such as schedulability and service guarantee for low-criticality applications.

==> relatedworks.tex <==



 % resource efficient mechanism~\cite{GU15} proposes a component based structure that tries to isolate each component, and hence when a single HC task exceed its LC execution estimate, other components are not influenced. The elastic mixed-criticality model allows for a flexible release pattern of LC tasks depending on the runtime resource consumption of HC tasks, essentially treating the LC workload as background~\cite{Su13,BuBa13,JZP13}.  This was improved by the service adaptation strategy that decreased the dispatch frequency of LC tasks only when a HC task violated its LC budget.







